HyperEnclave: An Open and Cross-platform Trusted Execution Environment

A number of trusted execution environments (TEEs) have been proposed by both academia and industry. However, most of them require specific hardware or firmware changes and are bound to specific hardware vendors (such as Intel, AMD, ARM, and IBM). In this paper, we propose HyperEnclave, an open and cross-platform process-based TEE that relies on the widely-available virtualization extension to create the isolated execution environment. In particular, HyperEnclave is designed to support the flexible enclave operation modes to fulfill the security and performance demands under various enclave workloads. We provide the enclave SDK to run existing SGX programs on HyperEnclave with little or no source code changes. We have implemented HyperEnclave on commodity AMD servers and deployed the system in a world-leading FinTech company to support real-world privacy-preserving computations. The evaluation on both micro-benchmarks and application benchmarks shows the design of HyperEnclave introduces only a small overhead.

==> files/enclave_sdk_backup.tex <==
\section{The enclave SDK}
%\subsection{Programming model}
\label{subsec:sgxprogramming}
\wenhao{maybe this section could be simplifed and put into Sec. 3}


\begin{table}[t]
    \caption[ABC]{SGX instructions supported in HyperEnclave.}
    \label{tab:sgx-instructions}
    \footnotesize\centering
    \begin{tabular}{ccll}
        \toprule
        S/U   & Type  & Instruction & Description \\
        \midrule
        S     & EXE   & \textsf{ECREATE }   & Create an enclave \\
        S     & MEM   & \textsf{EADD    }   & Add a 4K page \\
        S     & MEM   & \textsf{EEXTEND }   & Extend enclave measurement \\
        S     & MEM   & \textsf{EREMOVE }   & Remove a page from EPC \\
        S     & EXE   & \textsf{EINIT   }   & Initialize an enclave \\
        U     & EXE   & \textsf{EENTER  }   & Enter an enclave \\
        U     & EXE   & \textsf{EEXIT   }   & Exit an enclave \\
        U     & EXE   & \textsf{ERESUME }   & Re-enter an enclave \\
        U     & SEC   & \textsf{EGETKEY }   & Create a cryptographic key \\
        U     & SEC   & \textsf{EREPORT }   & Create a cryptographic report \\
        \bottomrule
    \end{tabular}
\end{table}

The enclave SDK is built upon the official SGX SDK. By replacing the SGX user leaf functions (e.g., \textsf{EENTER}, \textsf{EEXIT} and \textsf{ERESUME}) with hypercalls,
%\textsf{VMMCALL} instructions,
SGX programs can run on HyperEnclave with little or no source code changes. Once the enclave executes these user leaf functions, it traps to \visorname and \visorname emulates the functionalities of the corresponding SGX instructions. Table~\ref{tab:sgx-instructions} summarizes the SGX instructions supported in HyperEnclave. 

%and provides APIs compatible with the official Intel SGX SDK.


%Our Enclave SDK provide SGX SDK API compatible with SGX Apps. Once Enclave calls ENCLx primitives, it traps to hypervisor. Hypervisor provides functionalities of corresponding primitives. SGX Apps Developers only need to re-compile existing apps with minimal porting effort. Table \ref{tab:sgx-instructions} summarize all primitives that HyperEnclave supports.

The enclave is compiled as a trusted library of the application, while the application itself runs in the \untrustedos. The enclave life cycle is managed through the emulation of a set of privileged SGX instructions (i.e., \textsf{ECREATE}, \textsf{EADD}, \textsf{EINIT} etc.). To this end, the kernel module running in the \untrustedos provides similar functionalities by invoking \visorname through hypercalls, and exposes the functionalities to the applications by the \textsf{ioctl()} interfaces. By emulating the privileged SGX instructions, \visorname is responsible of the management of the enclave life cycle, as described below.

%---------------------- begin ignore
\ignore{
The enclave is compiled as a trusted library of the application, while the application itself runs in the untrusted guest OS. The guest kernel module provides functionalities similar to the privileged SGX instructions by invoking the hypervisor through \textsf{VMMCALL} instructions, and exposes the functionalities to the application by the \textsf{ioctl()} interfaces.
\textcolor{red}{The kernel module also maintains the enclave guest physical memory pool of the guest OS, such that all enclave guest physical pages are allocated in the pool. As such, the kernel module is still in charge of the virtual address to physical address mapping of enclave pages in the guest OS. To prevent address mapping attacks, the hypervisor maintains a data structure similar to the EPCM of SGX, which stores the the EPC page information, including the page type, permissions, the owner enclave, the page linear address and whether it is currently in use.}
By emulating the privileged SGX instructions, the hypervisor is responsible of the management of the enclave life cycle, as described below.
}
%-------------------- end of ignore

%为此我们实现了类似于 SGX 中的 EPCM (Enclave Page Cache Map) 结构，记录了每个 EPC 页面的权限、类型、所属的 enclave、以及是否正在被使用等信息。如果通过安全检查，就向 enclave VM 的 GPT 和 NPT 中添加该 EPC 页面的映射，并设置相应的权限。最后，HyperEnclave 会把页面内容从普通内存拷贝到 EPC 内存。

\mypara{Creation}
During enclave creation, the application creates the SECS (i.e., SGX Enclave Control Structure, and we use the same notation as SGX for simplicity) structure in normal memory, and invokes the kernel module using the \textsf{ioctl} interface. The kernel module creates an SECS page in the enclave memory pool and traps to the hypervisor to emulate the \textsf{ECREATE} instruction. Upon the request, the hypervisor creates an enclave instance by setting up a secure guest VM (i.e., the enclave VM) for the enclave. Then the hypervisor allocates a free EPC page for the SECS page\ignore{ to the enclave VM}, copies the SECS structure from normal memory to the EPC page, and marks the GVA of the SECS page as the enclave ID. The SECS structure in HyperEnclave is similar to that of SGX (see~\cite[Volume 3, Chap. 33.7]{IntelDevelopmentManual} for details), while we add the size of the marshaling buffer as an additional attribute.




%------------------- begin ignore
\ignore{
During enclave creation, the application invokes the kernel module with the \textsf{ioctl} interface. The kernel module creates a SECS (i.e., SGX Enclave Control Structure, and we use the same notation as SGX for simplicity) page in the enclave memory pool and passes the page address to invoke the emulated \textsf{ECREATE} instruction in the hypervisor. The hypervisor creates an enclave instance by setting up a secure guest VM (i.e., the enclave VM) and the NPT for the enclave. Then the hypervisor allocates a free EPC page for the SECS page to the enclave VM and marks the GPA of the SECS page as the enclave ID.\wenhao{ToDo: revise; the kernel module and the application use the GVA of SECS (same as SGX)} 
\shuang{Then the hypervisor allocates a free EPC page for the SECS page to the enclave VM, and the kernel module and the application use the GVA of SECS as enclave ID.}
The SECS structure in HyperEnclave is similar to that of SGX (see~\cite[Volume 3, Chap. 33.7]{IntelDevelopmentManual} for details), while we add the size of the marshaling buffer as an additional attribute.
}
%------------------- end of ignore

\mypara{Loading}
To load an enclave library, the application passes the enclave pages information, including the source page address and the enclave page's GVA, to the kernel module. The kernel module finds a free enclave guest physical page in the enclave memory pool, map it with the input GVA, and passes the pages information to invoke the emulated \textsf{EADD} instruction in \visorname. 
\visorname verifies that GVA is within the enclave linear address range (ELRANGE) and the enclave guest physical page is within the enclave memory region. Furthermore, it ensures that the guest physical page is not in use by other enclaves. Then \visorname copies the page content from the source page to the enclave page and add the mapping of the enclave's page to the enclave VM's NPT. \visorname also measures the enclave page content and attributes, then updates the measurement to the \textit{mrenclave} field of SECS. 

\mypara{Initialization}
After the enclave library is loaded to the EPC memory, the application invokes the emulated \textsf{EINIT} instruction in \visorname, passing the SIGSTRUCT structure as parameters. The SIGSTRUCT holds the enclave's measurement and other enclave attributes, and is signed by the enclave developer. \visorname verifies the signature and the enclave's measurement against the measurement stored in the SECS, and updates the SECS field if the verification passes.

%------------------- begin ignore
\ignore{After the enclave library is loaded to the EPC, the applications passes the SIGSTRUCT structure to the kernel module, and the kernel module invokes the  the emulated \textsf{EINIT} instruction in the hypervisor. The hypervisor verifies the SIGSTRUCT and updates the SECS field.\wenhao{ToDo: what is SIGSTRUCT and what kind of verification is performed} \shuang{Enclaves’ certificate is called SIGSTRUCT and is a mandatory supplement for launching any enclave. The SIGSTRUCT holds enclave’s MRENCLAVE together with other enclave attributes. SIGSTRUCTs are signed by the ISV with its private key, which was originally signed by an SGX launch authority.} Furthermore, the hypervisor adds the mapping of the marshalling buffer (see Sec.~\ref{sec:defense-against-mapping-attack}) to the enclave's guest page table.
}
%------------------- end of ignore


\mypara{Teardown}
After the enclave finishes the computation, the application notifies the kernel module to destroy the enclave by invoking the emulated \textsf{EREMOVE} instruction. \visorname removes the corresponding mappings from both the enclave's page table, and clears the enclave page's content before returning the page to the EPC. Then the kernel module removes the mappings in the normal VM and returns the enclave page to the enclave guest physical memory pool.

\mypara{Synchronous enclave entry and exiting}
The enclave thread is bound with a specific type of enclave pages, known as the Thread Control Structure (TCS) pages. The TCS pages are not directly accessible by the \untrustedos or the enclave.
After the enclave is initialized, the application can pass the TCS page address to invoke the emulated \textsf{EENTER} instruction. \visorname switches the VCPU state from the normal mode to the secure mode as follows. It saves the VCPU state of the normal mode, and fills the VCPU state from the TCS page. Specifically, it sets the instruction pointer to the value indicated by the OENTRY field in the TCS page. Last, it switches the GPT and NPT of the enclave and flushes the TLBs.

The enclave invokes the emulated \textsf{EEXIT} instruction in \visorname to return to the application. \visorname restores the VCPU state, switches the GPT and NPT to the \untrustedos and flushes the TLBs to switch the VCPU back to the normal mode.
%saved during \textsf{EENTER} and GPR (General purpose register) and FPR (Floating Point registers) are scrubbed then 

%enclave finishes initialization, untrusted app may issue \textsf{EENTER} in user mode to run enclave code. \textsf{EENTER} traps host mode. Hypervisor switch vcpu state from normal guest to secure guest mode. 

%To enforce integrity of enclave control flow, the entry of enclave, thread local storage address information are collected within a page called Thread Control Structure (TCS). The content of TCS is determined during compilation. During \textsf(EADD), TCS is written to enclave memory region and measured by hypervisor. Either Guest OS or Enclave can access the TCS page. 

%When switching to secure guest mode, hypervisor 1)save normal guest mode vcpu state 2)fills the vcpu state (RIP, TLS pointer) from selected TCS page. 3) switch GPT and NPT of enclave and flush TLB.

%Whenever enclave wants to run untrusted part code, it issues \textsf{EEXIT} in user mode and traps to host mode. Hypervisor restore the vcpu state saved during \textsf{EENTER} and GPR (General purpose register) and FPR (Floating Point registers) are scrubbed then vcpu switch back to normal guest mode.  

\mypara{Asynchronous Enclave Exit (AEX) and recovery}
To handle the interrupt and exception triggered in the enclave, \visorname configures the VCPU to trap all interrupts and exceptions to the \host. \visorname saves the enclave's context in the State Saving Area (SSA) of the TCS page, clears the registers to prevent information leakage and forwards the interrupt or exception to the normal VM. After the \untrustedos completes handling the interrupt or exception, the application invokes the emulated \textsf{ERESUME}
instruction in \visorname, which restores the enclave context from the SSA and resumes the execution of the enclave.

\mypara{Secret key generation}
When \visorname is initialized for the first time, it generates a root key $K_{root}$ from the random number generator (RNG) module of the TPM. $K_{root}$ is stored outside the TPM using TPM's seal operation. During the booting process on system reset, \visorname decrypts $K_{root}$ using TPM's unseal operation, which guarantees that $K_{root}$ can only be unsealed with the exactly same TPM chip with matching PCR configurations. Furthermore, \visorname floods the PCRs with a constant before transferring control to the \untrustedos to prevent it from retrieving $K_{root}$. All other key materials, including the enclave's sealing key and report key are derived from both $K_{root}$ and the enclave's measurement,
%(i.e., MRENCLAVE), 
and can be retrieved using the emulated instructions (i.e., \textsf{EGETKEY} and \textsf{EREPORT}) provided by \visorname.


%The data needs to be sealed in HyperEnclave is then encrypted using $K_{seal}$.  

%The enclave's key materials, including the 
%\shuang{Hypervisor derives the enclave's $K_{root}$ from $K_{seal}$ with enclave's \textit{mrenclave}. Enclave may obtain the $K_{root}$ through \textsf{EGETKEY}. }


%encrypt data using the storage root key (SRK) key in the TPM chip. In practice this means that data sealed with a TPM can only be unsealed (decrypted) with the exactly same TPM chip which binds the encryption to a specific device

%\wenhao{ToDo: using the TPM seal/unseal. As the TPM is shared with untrusted guest, during the boot process when the HyperEnclave is alive, it will unseal the key and flood the PCR to prevent the untrusted from retrieving the secret.}

%-----------------------------------------------------------------
\ignore{
Hypervisor在首次启动时， 会从tpm中获取256bit的随机数作为secret，并使用代表平台完整性配置的PCR（0-8，12和13）seal到tpm nv中。后继，Hypervisor每次启动时，unseal出该secret并保存在自己的内存中。当Enclave需要获取各种key（seal, report key等）时， hyperEnclave使用root secret和enclave自身的信息为其执行密钥derivation操作。此处由于TPM是共享的，一种潜在的攻击方式是Guest OS上的恶意应用可以在hypervisor启动并且对应的PCR寄存器被扩展之后调用TPM unseal命令获得HyperEnclave的secret，进而获取Enclave的机密数据。为了阻止这种攻击，hypervisor在完成secret的unseal之后，会扩展一个常数到PCR 12寄存器中，以淹没原来的PCR值。Hash函数的单向性确保恶意应用无法恢复PCR12原来的值。Hypervisor先于任何应用启动， 应用无法抢在hypervisor使用常数扩展PCR 12以便unseal secret。
}
%------------------------------------- ignore

%\mypara{Generating a cryptographic report of the enclave}
%\shuang{TODO}



%\textsf{ERESUME} and traps to host mode. Hypervisor restores the enclave context from SSA and resume enclave continue to run.

\mypara{Additional notes}
To be compatible with the SGX programming model, most data structures involved in HyperEnclave (such as the SIGSTRUCT structure, the SECS page and the TCS page) are similar to that of SGX. The details are omitted due to space constraints and we refer the readers to the SGX manual~\cite{IntelDevelopmentManual} for more information.

%\wenhao{we can briefly discuss the enclave's multi-threading support here}
With the HyperEnclave design, it is straightforward to support oversubscription of EPC pages in an enclave, since the EPC pages are managed by \visorname. Multi-threading within the enclave is supported by maintaining more than 1 TCS pages in the enclave. Exception handling within the enclave is supported by setting more than 1 SSA page for every TCS page. We omit the design details here.
 
%\shuang{App SDK maintains SECS/TCS context for each enclave thread. However, only Hypervisor can access the content of SECS/TCS of the enclave located in the isolated memory. The input params of \textsf{ENCLS} contains the enclave ID used by hypervisor to index the enclave. When invoke \textsf{ENCLU}, hypervisor queries the EPCM structure to find corresponding enclave from the GPA translated from input GVA within ELRANGE. Specifically, for \textsf{EENTER} and \textsf{EEXIT}, Hypervisor fills the enclave context from the corresponding TCS of this enclave thread. }

%-----------------------------------------------------------------
\ignore{
%when App creates an enclave, it pass SECS (SGX Enclave Control Structure) via mentioned ioctl and issues \textsf{ECREATE} in kernel module. This primitive invokes hypervisor and create an enclave instance. The GPA of SECS may be enclave ID. 

%When loading an Enclave image, the App pass enclave page information to kernel module. the latter find a free physical enclave page, map it with input GVA and issues \textsf{EADD}. 
%System traps host mode. hypervisor verifies whether 1) the GVA within enclave linear address (ELRANGE) and enclave page is within enclave memory region.  2) the enclave page is not allocated to other enclaves to defeat alias mapping attack (Figure \ref{fig:alias-mapping-attack}). 3) copy the source page content from normal memory to the isolated enclave memory region. 4) measures the enclave page content and attribute then extend to SECS field. 
%Adding and measure enclave page is time-consume task. it cannot finish in one instructions duration. To workaround such hardware limitation, SGX splits this process into two primitives \textsf{EADD} and \textsf{EEXTEND}. However, HyperEnclave can finish the all the tasks within one traps and it's more flexible than SGX. 
%5) Adding GVA to GPA mapping of enclave page in enclave guest page table (GPT) and GPA to HPA mapping in enclave nested page table (NPT).
%6) Memorize all GPA of enclave page belongs to this enclave.  

%With the help of the guest OS kernel module, the untrusted application invokes the hypervisor for enclave initialization and destroy

%take responsibility to invoke loading the trusted library.
%When an enclave is loaded, the hypervisor creates a 


%SGX enclave is a trusted library of corresponding App. The untrusted part of App take responsibility to invoke loading the trusted library. When running code with in Enclave, CPU switches to enclave mode. when running code outside enclave, CPU switches back to normal mode. 
%Enclave is created and loaded in isolated memory region by hypervisor incorporated with 
%untrusted app. 

%Normal guest mode does not have the mapping of enclave memory region in nested page table which is controlled by hypervisor. In this way, hypervisor enforces memory isolation between enclave and normal mode.  

%HyperEnclave leverages virtualization technology to create a secure guest mode. Hypervisor involved in every mode switch to guarantee vcpu context confidentiality and integrity. 
When running code within enclave, it traps to host mode. Hypervisor switches VCPU to secure guest mode and launches the Guest VM to run enclave. when running code outside enclave, cpu traps to host mode, hypervisor loads vcpu state as normal guest mode and Guest VM to run App. 
untrusted os creates and manages the enclave mapping. To thwart various mapping attack from malicious OS to archive memory integrity, SGX modify page missing handler (PMH) and extra EPCM (inverse mapping table) to track Enclave PA to VA mapping must be consistent with the state after enclave initialization. 

HyperEnclave solves this challenge without any hardware change. Hypervisor manages the guest page table of enclave and apply marshalling parameter buffer to limit data exchange between different mode. More details are presented in Sec.~\ref{sec:defense-against-mapping-attack})

\mypara{Enclave constructing and deconstructing}
SGX enclave life cycle is managed by \textsf{ENCLS} in privileged mode. HyperEnclave provides a kernel module to issues these primitives to hypervisor and exposes corresponding \textsf{ioctl()} interface to user mode. 

when App creates an enclave, it pass SECS (SGX Enclave Control Structure) via mentioned ioctl and issues \textsf{ECREATE} in kernel module. This primitive invokes hypervisor and create an enclave instance. The GPA of SECS may be enclave ID. 

%为此我们实现了类似于 SGX 中的 EPCM (Enclave Page Cache Map) 结构，记录了每个 EPC 页面的权限、类型、所属的 enclave、以及是否正在被使用等信息。如果通过安全检查，就向 enclave VM 的 GPT 和 NPT 中添加该 EPC 页面的映射，并设置相应的权限。最后，HyperEnclave 会把页面内容从普通内存拷贝到 EPC 内存。

During Enclave initialization, Apps inputs SIGSTRUCT structure via kernel module. kernel module issues \textsf{EINIT} and traps host mode. hypervisor 1) verifies the SIGSTRUCT and update the SECS field.  2) Add masharshalling buffer mapping to enclave GPT. (detail in Section \ref{sec:defense-against-mapping-attack}).


App closes the the file handle of kernel module to notify it destroy the enclave. the kernel module issue \textsf{EREMOVE} and traps to host mode. Hypervisor 1) Iterate all enclave entry in EPM and remove corresponding mapping from enclave GPT and NPT. 2) scrub enclave page content before return to enclave memory pool. After return to kernel module, it remove the mapping in App Guest page table and return the enclave page to enclave memory pool. 

\mypara{Enclave entry and exiting}
After enclave finishes initialization, untrusted app may issue \textsf{EENTER} in user mode to run enclave code. \textsf{EENTER} traps host mode. Hypervisor switch vcpu state from normal guest to secure guest mode. 

To enforce integrity of enclave control flow, the entry of enclave, thread local storage address information are collected within a page called Thread Control Structure (TCS). The content of TCS is determined during compilation. During \textsf(EADD), TCS is written to enclave memory region and measured by hypervisor. Either Guest OS or Enclave can access the TCS page. 

When switching to secure guest mode, hypervisor 1)save normal guest mode vcpu state 2)fills the vcpu state (RIP, TLS pointer) from selected TCS page. 3) switch GPT and NPT of enclave and flush TLB.

Whenever enclave wants to run untrusted part code, it issues \textsf{EEXIT} in user mode and traps to host mode. Hypervisor restore the vcpu state saved during \textsf{EENTER} and GPR (General purpose register) and FPR (Floating Point registers) are scrubbed then vcpu switch back to normal guest mode.  

\mypara{Asynchronous Enclave Exit (AEX)}
To handle the interrupt or exception triggered in the enclave, instead of running a guest OS to proceed privileged events in secure guest mode, the hypervisor configures the VCPU to trap all interrupts and exceptions to host mode. The HyperEnclave hypervisor saves the enclave context in an enclave page called SSA (State Save Area), clears the registers to prevent information leakage and forwards the interrupt or exception to the guest VM. After the guest VM completes handling the interrupt or exception, untrusted part of App is scheduled to run. it issues \textsf{ERESUME} and traps to host mode. Hypervisor restores the enclave context from SSA and resume enclave continue to run.


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/alias-mapping.pdf}
        \caption{Alias mapping attack}
%        \Description{Alias mapping attack}
        \label{fig:alias-mapping-attack}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/remapping.pdf}
        \caption{Remapping attack}
%        \Description{Remapping attack}
        \label{fig:remapping-attack}
    \end{subfigure}
    \caption{\textbf{Potential mapping attacks on HyperEnclave.} (a) 两个不同 enclave 中的虚拟地址被映射到同一 EPC 页面。(b) 一个 enclave 中，非 ELRANGE 范围内的虚拟地址被映射到 EPC 页面。}
    \label{fig:mapping-attack}
\end{figure*}

%------------------------------------- ignore

\subsection{Defense Against Mapping Attack}\label{sec:defense-against-mapping-attack}

1) Enclave needs to exchanges data with untrusted part of App. Enclave and App shares the same memory address space. SGX allows CPU in enclave mode to access normal memory of untrusted part of App arbitrarily. 
2) untrusted OS controls the enclave/App's page table. it may initiate mapping attack by manipulating the memory mapping of enclave. (Figure \ref{fig:remapping-attack}).
3) SGX hardware modifies PMH (page missing handler) and add inverted page table (EPCM) to defeat various mapping attack. 

To thwart mapping attack, HyperEnclave have two challenges: 

\begin{itemize}
    \item \textbf{C-1:} \textit{How to synchronize enclave and app's memory view}.
    \item \textbf{C-2:} \textit{How to guarantee the integrity of enclave address translation} that means: in Enclave virtual memory view, the GVA within ELRANGE must map to a GPA inside the enclave memory range. the GVA outside ELRANGE must map to GPA outside enclave memory region. 
\end{itemize}

In order to solve \textbf{C-1}, one candidate solution is that enclave uses app's normal memory region mapping. however, this mapping is still controlled by untrusted guest OS which leads to mapping attack. 
To resolve \textbf{C-2}, one possible solution is trap base page table management. Enclave and App shares the same GPT(guest page table) which created by Guest OS. Hypervisor make this GPT write protected. Any update to the GPT traps to host mode. Hypervisor verifies whether  this update is correct or not. However, guest OS may update guest page table very often. Moreover, whenever hardware updates A/D bit of PTE, it also traps to host mode. This approach can fulfill the requirements but imposes big performance overhead and hypervisor needs to emulate A/D bit update and add implementation complexity. 

\mypara{Hypervisor-managed enclave guest page table}

% TODO: move to implementation 
当创建 enclave 时，guest OS 会在普通内存上为每个 enclave 都分配一段独立的 marshalling buffer，且这段内存 GVA 到 GPA 的映射关系是固定的，不能再被修改，也不能被换出。然后通过 \textsf{EINIT} hypercall 传入 marshalling buffer 基址和大小，HyperEnclave 将这段内存的映射添加进 enclave 的 GPT 和 NPT 中，只设置读写属性，而不能被执行。当 enclave 初始化完毕，使用 ECALLs 或 OCALLs 跨越安全边界调用 enclave 或不可信 app 的函数时，函数的参数需要被整顿，然后从普通内存或 EPC 内存拷贝到 marshalling buffer，使得被调用者可以访问。这些操作都在 App SDK 中实现，对于 SGX 应用来说是透明的，无需为此修改源码。

HyperEnclave design an innovative solution to mitigate these challenges:
1) Limit Enclave's capability to access normal memory. HyperEnclave pre-allocates an share memory named \textbf{marshalling buffer} in normal memory(Figure: \ref{fig:memory-view}). All data exchanged between enclave and app must pass through the marshalling buffer. 
2) The mappings of marshalling buffer is fixed during the whole enclave life cycle by pre-populate the physical memory and pin it in memory. 
3) During Enclave creation, hypervisor create a new GPT/NPT for enclave VM in hypervisor owned memory. 
3) During Enclave initialization, app passes the start GVA and size of marshalling buffer to hypervisor through \textsf{EINIT} primitive. Hypervisor verify this GVA and length is outside ELRANGE then add these mappings to enclave GPT/NPT with RW attributes only. 

In our design, Hypervisor only allows Enclave to access its own enclave memory and marshalling buffer. After Enclave initialization, all memory mappings of the enclave is deterministic and not changed until enclave is destroyed. It does not need to sync virtual memory view of enclave and app anymore. (resolve \textbf{C-1}). For Enclave's GPT/NPT are sit in hypervisor's memory which maps to the empty page in Guest VM. Malicious guest OS cannot change the mapping of enclave.  (resolve \textbf{C-2})

This design bring more benefits: 
1) All enclave mapping are deterministic after enclave initialization. No page fault during enclave running to boost enclave performance. Closing page table based side channels~\cite{xu2015controlled,wang2017leaky,van2017telling}. 
2) enclave is limited to access App's normal memory and raise the bar for enclave to attack guest VM. 
3) Compare with SGX design, HyperEnclave does not need to modify hardware and much easier to deploy.

% TODO: check rip & rsp on EEXIT to enforce eexit control flow integrity
SGX allows Enclave to access the whole App's memory address from enclave mode and jump to arbitrary RIP of App through \textsf{EEXIT} when CPU goes back to normal mode.
}
%---------------------------- end of ignore
